On Two Infinite Families of Pairing Bijections

We describe two general mechanisms for producing pairing bijections (bijective functions defined from N x N to N). The first mechanism, using n-adic valuations results in parameterized algorithms generating a countable family of distinct pairing bijections. The second mechanism, using characteristic functions of subsets of N provides 2^N distinct pairing bijections. Mechanisms to combine such pairing functions and their application to generate families of permutations of N are also described. The paper uses a small subset of the functional language Haskell to provide type checked executable specifications of all the functions defined in a literate programming style. The self-contained Haskell code extracted from the paper is available at http://logic.cse.unt.edu/tarau/research/2012/infpair.hs .

==> TOOLS/chheader12.tex <==
\usepackage{graphicx}
%\usepackage{subfig} % creates problems - fails maketitile
\usepackage{url}
\usepackage{verbatim}
\usepackage{color}
\definecolor{lgray}{gray}{0.92}
\definecolor{lblue}{rgb}{0.90,0.90,1.00}
\definecolor{lyellow}{rgb}{1.00,1.00,0.70}

\usepackage{listings}
\lstloadlanguages{Haskell}
% parameters in this will be overriden by same for {code}
% so this will look the same - except that it will not be treated as code

\newenvironment{codex}{\small\verbatim}{\endverbatim\normalsize}
\let\codeh\comment 

\lstnewenvironment{code}
    {\lstset{}%
      \csname lst@SetFirstLabel\endcsname}
    {\csname lst@SaveFirstLabel\endcsname}
    \lstset{
      basicstyle=\small\ttfamily,
      %frame=single, 
      backgroundcolor=\color{lgray},
      flexiblecolumns=false,
      basewidth={0.5em,0.45em},
      literate={+}{{$+$}}1 {/}{{$/$}}1 {*}{{$*$}}1 {=}{{$=$}}1
               {>}{{$>$}}1 {<}{{$<$}}1 {\\}{{$\lambda$}}1
               {\\\\}{{\char`\\\char`\\}}1
               {->}{{$\rightarrow$}}2 {>=}{{$\geq$}}2 {<-}{{$\leftarrow$}}2
               {<=}{{$\leq$}}2 {=>}{{$\Rightarrow$}}2 
               {>>}{{>>}}2 {>>=}{{>>=}}2
               {|}{{$\mid$}}1
    }
\newtheorem{prop}{Proposition}
\newtheorem{conj}{Conjecture}
\newtheorem{fact}{Fact}
\newtheorem{df}{Definition}
\newtheorem{lem}{Lemma}
\newtheorem{ex}{Example}
\newcommand{\BI}[0]{\begin{itemize}}
\newcommand{\EI}[0]{\end{itemize}}
\newcommand{\I}[0]{\item}
\newcommand{\BE}[0]{\begin{enumerate}}
\newcommand{\EE}[0]{\end{enumerate}}
\newcommand{\PP}[0]{ \vskip 0.6cm }
\newcommand{\BX}[0]{\begin{codex}}
\newcommand{\EX}[0]{\end{codex}}
\newcommand{\BV}[0]{\begin{verbatim}}
\newcommand{\EV}[0]{\end{verbatim}}

\newcommand{\colorON}{\lstset{backgroundcolor=\color{yellow}}}
\newcommand{\colorOFF}{\lstset{backgroundcolor=\color{white}}}
    
\def \bscale1 {0.25}
\def \bscale {0.25}
\def \N {\mathbb{N}}

% \FIG{Label}{Title}[scale]{file.suf}
\newcommand{\FIG}[4]{
\begin{figure}[htbp]
\centering
{\includegraphics[scale=#3]{figs/#4}}
\caption{#2}
\label{#1}
\end{figure}
}

% \FIG{Label}{Title}[scale]{file.suf}
\newcommand{\CFIG}[4]{
\begin{figure}[htbp]
\centering
{\includegraphics[scale=#3,viewport=100 100 500 500,clip]{figs/#4}}
\caption{#2}
\label{#1}
\end{figure}
}
% totalheight=0.4\textheight

% \HFIGS{Label}{Title}{Title1}{Title2}{PNG1}{PNG2}
\newcommand{\HFIGS}[6]{
\begin{figure}[htbp]
  \centering
  \subfloat[#3]{
    {\includegraphics[scale=0.60]{figs/#5}}}   
  \subfloat[#4]{
    {\includegraphics[scale=0.60]{figs/#6}}}
  \caption{#2}
  \label{#1}
\end{figure}
}

% \VFIGS{Label}{Title}{Title1}{Title2}{PNG1}{PNG2}
\newcommand{\VFIGS}[6]{
\begin{figure}[htbp]
  \begin{center}
    {\includegraphics[scale=0.40]{figs/#5}}
    {\includegraphics[scale=0.40]{figs/#6}}
  \caption{#2: {\em #3} and {\em #4}}
  \label{#1}
  \end{center}
\end{figure}
}


% \VSFIGS{Label}{Title}{Title1}{Title2}{PNG1}{PNG2}{Scale}
\newcommand{\VSFIGS}[7]{
\begin{figure}[htbp]
  \begin{center}
    {\includegraphics[scale=#7]{figs/#5}}
    {\includegraphics[scale=#7]{figs/#6}}
  \caption{#2 #3 #4}
  \label{#1}
  \end{center}
\end{figure}
}



